Observation of WZ Production

We report the first observation of the associated production of a W boson and a Z boson. This result is based on 1.1 fb-1 of integrated luminosity from ppbar collisions at sqrt{s} = 1.96 TeV collected with the CDF II detector at the Fermilab Tevatron. We observe 16 WZ candidates passing our event selection with an expected background of 2.7 +/- 0.4 events. A fit to the missing transverse energy distribution indicates an excess of events compared to the background expectation corresponding to a significance equivalent to six standard deviations. The measured cross section is sigma(ppbar -> WZ) = 5.0^{+1.8}_{-1.6} pb, consistent with the standard model expectation.

==> WZ_systematics.tex <==
\begin{table}
\caption{Systematic uncertainties as a percentage of the expected
yield in the signal region in 1.1 ${\rm fb}^{-1}$.}
\label{tbl:syst}
\begin{ruledtabular}
\begin{tabular}{lrrrr}
         Variation          &           $ZZ$               &           $Z\gamma$          &           $t\bar{t}$         &           $WZ$               \\
\hline \hline
Expected Yield                     &       0.9               &       0.5               &       0.1               &       9.8             \\
\hline
Lepton Id Efficiency         &             2.0\%      &             1.9\%   &             1.2\%   &             1.9\% \\
Trigger Efficiency           &             0.6\%      &             0.9\%   &             0.4\%   &             0.6\% \\
$\MET$ Modeling              &             1.0\%      &            25.0\%   &             1.0\%   &             1.0\% \\
Energy Scale                 &             1.0\%      &             1.0\%   &             -           &             1.0\% \\
PDF Uncertainty              &             2.0\%      &             2.0\%   &             2.0\%   &             2.0\% \\
Cross-Section                &            10.0\%      &            20.0\%${}^{*}$   &            10.0\%   &             -         \\
\hline
Total                        &                 10.5\%   &                 32.2\%   &                 10.3\%   &                  3.2\% \\
\end{tabular}
${}^{*}$ includes conversion and material description systematics.
\end{ruledtabular}
\end{table}

